A case for using rotation invariant features in state of the art feature matchers

The aim of this paper is to demonstrate that a state of the art feature matcher (LoFTR) can be made more robust to rotations by simply replacing the backbone CNN with a steerable CNN which is equivariant to translations and image rotations. It is experimentally shown that this boost is obtained without reducing performance on ordinary illumination and viewpoint matching sequences.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/Standard_All_MMA_triple.tex <==
\begin{tabular}{llll}
\toprule
\multicolumn{1}{r}{MMA} &                                               @3px &                                               @5px &                                              @10px \\
\midrule
LoFTR (re-evaluated) &     {\small(93.4, \phantom{00.0}, \phantom{00.0})} &     {\small(95.2, \phantom{00.0}, \phantom{00.0})} &     {\small(96.1, \phantom{00.0}, \phantom{00.0})} \\
LoFTR (re-trained)   &                         {\small(93.4, 93.8, 93.3)} &                         {\small(95.1, 95.4, 95.0)} &                         {\small(96.0, 96.3, 95.9)} \\
SE2-LoFTR-4          &                         {\small(94.3, 94.5, 94.1)} &                         {\small(96.2, 96.4, 96.0)} &                         {\small(97.3, 97.5, 97.0)} \\
SE2-LoFTR-4-Big      &                         {\small(94.5, 94.7, 94.2)} &                         {\small(96.5, 96.7, 96.2)} &                         {\small(97.5, 97.6, 97.2)} \\
SE2-LoFTR-8          &                         {\small(94.1, 94.1, 94.0)} &                         {\small(96.1, 96.2, 96.0)} &                         {\small(97.3, 97.4, 97.2)} \\
\bottomrule
\end{tabular}

